Directional Bias Amplification

Mitigating bias in machine learning systems requires refining our understanding of bias propagation pathways: from societal structures to large-scale data to trained models to impact on society. In this work, we focus on one aspect of the problem, namely bias amplification: the tendency of models to amplify the biases present in the data they are trained on. A metric for measuring bias amplification was introduced in the seminal work by Zhao et al. (2017); however, as we demonstrate, this metric suffers from a number of shortcomings including conflating different types of bias amplification and failing to account for varying base rates of protected attributes. We introduce and analyze a new, decoupled metric for measuring bias amplification, $\text{BiasAmp}_{\rightarrow}$ (Directional Bias Amplification). We thoroughly analyze and discuss both the technical assumptions and normative implications of this metric. We provide suggestions about its measurement by cautioning against predicting sensitive attributes, encouraging the use of confidence intervals due to fluctuations in the fairness of models across runs, and discussing the limitations of what this metric captures. Throughout this paper, we work to provide an interrogative look at the technical measurement of bias amplification, guided by our normative ideas of what we want it to encompass. Code is located at https://github.com/princetonvisualai/directional-bias-amp

==> Input_Files/Existing_Metrics_OLD.tex <==
\olga{I shared the other overleaf doc with you, can you please save this and incorporate the new ones (incl. the new section title here)}


% In Sec.~\ref{sec:error_types} we begin by presenting existing fairness metrics and showing how bias amplification can distinguish errors resulting from under- and overclassification in a way that others cannot; in Sec.~\ref{sec:biasamptheirs} we discuss some shortcomings of \biasamptheirs{}; in Sec.~\ref{sec:our_metrix_exp} we present our metric, \biasampours{}, which addresses the shortcomings noted in the previous section, with experiments in Sec.~\ref{sec:empirical_benefits}; we conclude in Sec.~\ref{sec:ta_bias} with a discussion about predicting sensitive attributes.

We present existing fairness metrics and show how bias amplification can distinguish errors resulting from under- and overclassification in a way that others cannot, followed by a discussion of the shortcomings of \biasamptheirs{}.

\subsection{Problem Formulation and Notation}
We consider again the example from Fig.~\ref{fig:fig1}, where we want to classify a task, $T_t$, and an attribute, $A_a$. An image containing a woman is denoted by the presence of a binary indicator variable, $A_0=1$, or for notational convenience, simply $A_0$. On this dataset women ($A_0$) are correlated with painting ($T_0$), and men ($A_1$) with not painting ($T_1$). The set of attributes, $a\in\mathcal{A}=\{0, 1\}$ in this example, corresponds to $A_0$ and $A_1$, each of which is a binary indicator variable. When we introduce our proposed metric in Sec.~\ref{sec:our_metrix_exp}, this notation expresses our explicit and deliberate allowance for situations in which a person may identify with zero, one, or more than one attributes. The set of tasks, $t\in\mathcal{T}=\{0, 1\}$ in this example, follows a similar formulation to allow for multi-label settings. We imagine $N$ images each of $(A_0,T_0)$ and $(A_1,T_1)$ but only $N/2$ images of $(A_0,T_1)$ and $(A_1,T_0)$. A classifier trained to recognize painting on this data is likely to learn these associations and over-predict painting on images of women and under-predict painting on images of men; however, algorithmic interventions may counteract this and in fact result in the opposite behavior. 
% We formulate these in this way to establish uniformity in notation across the different metrics. 

\subsection{Overview of Existing Fairness Metrics}
\label{sec:error_types}

We begin with a review of existing fairness metrics in a concrete classification setting. 
Four fairness metrics we consider are: {\it False Positive Rate (FPR) and True Positive Rate (TPR) difference:} the difference in false positive (true positive) rate of predicting the label $T_0$ on images of $A_1$ versus $A_0$~\citep{chouldechova2016recidivism, hardt2016equalopp}, {\it accuracy difference:} difference between the task prediction accuracy on images of $A_1$ versus on images of $A_0$~\citep{berk2017risk}, and {\it mean accuracy across subgroups:} mean task prediction accuracy across the four image subgroups ($(A_0, T_0), (A_1, T_0), (A_0, T_1), \text{and } (A_1, T_1)$)~\citep{buolamwini2018gendershades}.
Fig.~\ref{fig:metric_comp} shows the behavior of fairness metrics under varying amounts of learned amplification. 
However, these four metrics are not designed to account for the training correlations, and unable to distinguish between cases of increased or decreased learned correlations. %, motivating a need for a measurement that can: bias amplification.

\cite{zhao2017menshop} introduced an alternative to these that explicitly captures the notion of bias amplification. Concretely, they consider $P(A_a=1|T_t=1)$ of the training data as the fraction of times a protected attribute $A_a \in \mathcal{A}$ appears on images corresponding to task $T_t \in \mathcal{T}$. They then compare this with the test-time predictions made by the model, $P(\hat{A}_a=1|\hat{T}_t=1)$, or the number of times attribute $A_a$ is predicted on images where the task is predicted as $T_t$, which allows them to measure bias amplification in the absence of any additional annotations on the hold-out set. Note that in this formulation they are assuming the model is making predictions for both the task and the attribute. The full bias amplification metric (reformulated in our terms), is
% with $t\in\mathcal{T}$ as the tasks, and $a\in\mathcal{A}$ as the attributes: 
% is computed as 
% \biasamptheirs{} =
\begin{multline}
% \begin{split}
         \text{\biasamptheirs}=
         \frac{1}{|\mathcal{T}|}
     \sum_{t=1}^{|\mathcal{T}|} \sum_{a=1}^{|\mathcal{A}|} \underbrace{\mathbbm{1}\left( P(A_a=1|T_t=1) > \frac{1}{|\mathcal{A}|}\right)}_{y(t, a)}
   \\  \underbrace{\left ( P(\hat{A}_a=1|\hat{T}_t=1) - P(A_a=1|T_t=1)  \right )}_{\Delta(t, a)}
% \end{split}
\label{eqn:menshop}
\end{multline}
%  \begin{align}
%     %  \text{\biasamptheirs} &=\\
%      \frac{1}{|\mathcal{T}|}
%      \sum_{t=1}^{|\mathcal{T}|} \sum_{a=1}^{|\mathcal{A}|} &\underbrace{\mathbbm{1}\left( P(A_a=1|T_t=1) > \frac{1}{|\mathcal{A}|}\right)}_{y(t, a)}\\&
%      \underbrace{\left ( P(\hat{A}_a=1|\hat{T}_t=1) - P(A_a=1|T_t=1)  \right )}_{\Delta(t, a)}
% \label{eqn:menshop}
%  \end{align}
 
Fig.~\ref{fig:metric_comp} empirically demonstrates that this metric is able to capture the level of increasing bias amplification. (For consistency in comparison with prior metrics, we assume the model always correctly predicts the protected attribute $A$.) However, as we discuss in the next section, there are some properties of bias amplification that this metric is not able to capture: for example, it does not distinguish between errors in predicting the protected attribute versus errors in predicting the task. Thus we introduce a new metric (last graph of Fig.~\ref{fig:metric_comp}) which maintains the desirable properties from \cite{zhao2017menshop} while including a number of innovations.  



\begin{figure}[t]
\centering
\begin{subfigure}{}
\includegraphics[width=1.\linewidth]{Images/metric_comp.png} 
\end{subfigure}
\caption{\label{fig:metric_comp}
Different fairness metrics vary in how they respond to model errors. In our image dataset (Fig.~\ref{fig:fig1}) of predicting someone who is a woman or man to be painting or not, we consider a classifier that always predicts the task correctly for men, but varies for women. The x-axes of the graphs correspond to the fraction of women predicted to be painting, where the ground-truth is $2/3$, and the model does not predict false positives before this point. The first two metrics, FPR and TPR difference, only capture one of under- or overclassification. The next two metrics are symmetric around $2/3$, being unable to differentiate under- or overclassification. Both bias amplification metrics are able to distinguish between under- and overclassification.
% Different fairness metrics respond differently to model errors. Consider an image dataset (Fig~\ref{fig:1}) with the target task of predicting whether a person, who is a man or woman, in the image is painting or not painting. Consider a classifier which always makes the correct prediction on images with women, but over- or under-classifies the images with men as painting. In the graphs above, the x-axes correspond to the fraction of men predicted to be painting on the test dataset; further suppose that $1/3$ of the images with men are in fact painting, and the model never makes false-positive predictions.  The first 2 metrics, FPR and TPR difference each only capture one aspect of either under- or overclassification. The next 3 metrics are all symmetric around $1/3$, being unable to distinguish between under- or overclassification. Our proposed bias amplification metric (rightmost graph; Sec.~\ref{XX}) is designed to distinguish between under- and overclassification.
%How 6 different fairness metrics change as a function of the fraction of $a_2$ classified as $t_1$, where $1/3$ is the ground-truth. The first 2 metrics, FPR and TPR difference each only capture one aspect of either under- or overclassification, and even together, do not tell you whether the bias that is happening is in the direction of that in the training data, or opposite. The next 3 metrics are all symmetric around $1/3$, being unable to distinguish between under- or overclassification. Bias amplification is the only perspective that can properly distinguish under- and overclassification.
}
\end{figure}

% To analyze the shortcomings of existing fairness metrics, we consider the image classification dataset presented in Fig.~\ref{fig:fig1}. Further suppose there are N images each of $(a_1, t_1)$ and $(a_2, t_2)$ and only $\frac{N}{2}$ each of $(a_1, t_2)$ and $(a_2, t_1)$.
% Consider first two classifiers, C1 and C2, where one fails to recognize the atypical case $(t_1,a_2)$ and another that in contrast overestimates the prevalence of the atypical case $(t_2,a_1)$.  Concretely, suppose both classifiers are able to perfectly predict $a_1$ versus $a_2$, but C1 misclassifies $t_1$ as $t_2$ on images with $a_2$ half the time and C2 misclassifies $t_1$ as $t_2$ on images with $a_1$ half the time. Intuitively, C1 exhibits bias amplification whereas C2 overcompensates for it; proper fairness metrics need to distinguish between the two cases yet fail to do so: e.g., the mean accuracy across subgroups\footnote{equation}~\cite{XXX} of both is $0.88$ and the False Positive Rate difference\footnote{equation}~\cite{XXX} of both  is $0$. 
% In Fig.~\ref{fig:metric_comp} we vary the fraction of men ($a_2$) that are predicted to be painting ($t_1$), and show 5 fairness metrics in blue:


\subsection{Shortcomings of BiasAmp$_{\textnormal{MALS}}$}
\label{sec:biasamptheirs}

Despite the advantages of \biasamptheirs{} (Eqn.~\ref{eqn:menshop}) and its ability to distinguish under- and overclassifications of training correlations, this metric also suffers from a number of shortcomings. To ground our discussion, we will work directly with the model outputs released by~\citet{zhao2017menshop} from their Conditional Random Field (CRF) model on COCO~\citep{lin14coco}, which has predictions for gender and objects detected for each image.  
\subsubsection{Non-binary attributes}
\label{sec:nonbinary}
The first shortcoming is the metric assumes the protected attributes are binary, limiting its use: the indicator variable $y(t,a)$ only counts an increase in positive correlations, but not a decrease in negative correlations, in multi-attribute scenarios. 
% $A_a\in \mathcal{A}$ to be associated with every task $T_t\in \mathcal{T}$. 
Consider a task $T_0$ such that $A_0$ is associated with it, but none of the other $A_i$, where $i\in\mathcal{A}, i\neq 0$. In this scenario, $\Delta(T_0, A_i)$ is only measured when there is one other $A_i$ such that $A_i=\lnot A_0$, since $\Delta(t, a)=-\Delta(t, \lnot a)$.
% Consider a task $t\in\mathcal{T}$ and a binary protected attribute with values $a$ and $\lnot a$. The current contribution to \biasamptheirs can be rewritten as $diff(t,a)y(t,a)+(-diff(t,a)(1-y(t,a))$ since $diff(t,a)=-diff(t,\lnot a)$. 
A simple addition of $-\Delta$ 
% for all $A_i$'s 
when $y$ is 0 would count all bias amplification when there are more than two groups.
% ensures that when there are more than two groups, their bias amplification is also counted.

\subsubsection{Base rates}
\label{sec:baserates}
The second shortcoming is that the metric does not take into account the base rates of each attribute. Concretely, when determining in $y(t,a)$ of Eqn.~\ref{eqn:menshop} whether the attribute $A_a$ is correlated with the task $T_t$, $P(A_a=1|T_t=1)$ is compared to $\frac{1}{|\mathcal{A}|}$. However, this assumes that all $A_a$'s within $\mathcal{A}$ are evenly distributed, which may not be the case. For example, in COCO there are about 2.5x as many men as women, so it would appear that most objects positively correlate with men simply by nature of there being an overrepresentation of men. Consider the object \texttt{oven}; \biasamptheirs{} calculates $P(A_{\texttt{man}}=1|T_{\texttt{oven}}=1)=0.56>\frac{1}{2}$ and thus considers this object to be correlated with men rather than women. However, computing $P(A_{\texttt{man}}=1,T_{\texttt{oven}}=1) =  0.0103 < 0.0129 = P(A_{\texttt{man}}=1)P(T_{\texttt{oven}}=1)$
%$P(T=\texttt{oven}|A=\texttt{man}) = .0047 < .0056 = P(T=\texttt{oven})$
reveals that men are in fact \emph{not} correlated with oven, and the seeming overrepresentation comes from the fact that men are overrepresented in the dataset more generally. Not surprisingly, the model trained on this data learns to associate women with ovens and underpredicts men with ovens at test time, i.e., $P(\hat{A}_{\texttt{man}}=1 | \hat{T}_{\texttt{oven}}=1) -  P(A_{\texttt{man}}=1 | T_{\texttt{oven}}=1) = -0.10$. \biasamptheirs{} erroneously counts this as \emph{negative} bias amplification. 


\subsubsection{Entangling directions}
\label{sec:sub_disentangle}
Another shortcoming is the inability to distinguish between different \emph{types} of bias amplification. \citet{zhao2017menshop} discovers that ``Technology oriented categories
initially biased toward men such as \texttt{keyboard}... have each increased their bias toward
males by over 0.100." Concretely, from Eqn.~\ref{eqn:menshop}, $P(A_{\texttt{man}}=1|T_{\texttt{keyboard}}=1) = .70$ and $P(\hat{A}_{\texttt{man}}=1|\hat{T}_{\texttt{keyboard}}=1) = .83$, demonstrating an amplification of bias. However, the \emph{direction} or cause of bias amplification remains unclear: is the presence of man in the image increasing the probability of predicting a keyboard, or vice versa? Looking more closely at the model's disentangled predictions, we see that when conditioning on the attribute, $P(\hat{T}_{\texttt{keyboard}}=1|A_{\texttt{man}}=1)  = 0.0020 < 0.0032 =  P(T_{\texttt{keyboard}}=1|A_{\texttt{man}}=1)$, and when conditioning on the task, 
$P(\hat{A}_{\texttt{man}}=1|T_{\texttt{keyboard}}=1)  = 0.78 &> 0.70 =  P(A_{\texttt{man}}=1|T_{\texttt{keyboard}}=1)$,
% \begin{align}
%  P(\hat{T}=\texttt{keyboard}|A=\texttt{man})  = 0.0020 &< 0.0032 =  P(T=\texttt{keyboard}|A=\texttt{man}) \\
%  P(\hat{A}=\texttt{man}|T=\texttt{keyboard})  = 0.78 &> 0.70 =  P(A=\texttt{man}|T=\texttt{keyboard})
% \end{align}
indicating that keyboards are under-predicted on images with men yet men are over-predicted on images with keyboards. Thus the root cause of this amplification appears to be in the gender predictor rather than the object detector. Such disentangement allows us to properly focus algorithmic intervention efforts.
% not in basing the object prediction on the gender in the image (in fact, the model is \emph{less} likely to predict keyboard on images with men than would be expected given the training frequencies). It actually appears that the \emph{gender} prediction in images is heavily based on the presence of different objects (likely because gender is not a visually discriminative feature).  We observe a similar pattern in XX of the YY objects in the COCO dataset.
% This implies three things. First, the key concerns about object detectors learning to rely on gender features appear to be unfounded in this context. Second, it again brings up an important normative point we will discuss later regarding whether gender (and similar sensitive protected attributes) should be predicted at all. It appears that in this context predicting gender led to a potentially erroneous conclusion regarding the influence of gender on object detection, whereas in fact the core issue stemmed from attempting to predict gender in a context where gender features were not sufficiently discriminative -- and, where gender prediction was likely not necessary in the first place. 
This also highlights the need to consider the ground truth labels in addition to the predictions on the hold-out set, since when considering only the predictions, it is impossible to decouple the different sources of bias. 

\subsection{Threshold}
We fully replicate the original experiment from~\citet{zhao2017menshop} using \biasamptheirs{} on their model predictions and measure $.040$. However, we observe that ``man" is being predicted at a higher rate (75.6\%) than is actually present (71.2\%).
With this insight, we tune the decision threshold on the validation set such that the gender predictor is well-calibrated to be predicting the same percentage of images to have men as
% \begin{wrapfigure}{l}{0.3\textwidth}
% \vspace{-10pt}
%     \centering
%     \includegraphics[width=0.3\textwidth]{Images/biasamp_by_prop.png}
%     \caption{\label{fig:byprop}Bias amplification varying as a function of proportion of images classified to be men (controlled by classification threshold).}
% \vspace{-5pt}
% \end{wrapfigure}
the dataset actually has. When we calculate \biasamptheirs{} on these newly thresholded predictions for the test set, we see bias amplification drop from $0.040$ to $0.001$ just as a result of this threshold change, outperforming even the solution proposed in \citet{zhao2017menshop} of corpus-level constraints, which achieved a drop to only $0.021$. Fairness can be quite sensitive to the threshold chosen~\citep{chen2020threshold}, so careful threshold selection should be done, rather than using a default of $.5$.
% In Fig.~\ref{fig:byprop} we show how the amount of bias amplification, as measured by \biasamptheirs{} and \biasampoursTA{}, changes as we vary the threshold, i.e., proportion of people classified to be a man. We can see that when the threshold is chosen to be the one well-calibrated on the validation set rather than the default threshold, bias amplification is measured to be closer to zero for both metrics. 
When a threshold is needed in our experiments, we pick it to be well-calibrated on the validation set. Although we do not take this approach, because at deployment time it is often the case that discrete predictions are required, one could also imagine integrating bias amplification across proportion or threshold to have a threshold-agnostic measure of bias amplification, similar to what is proposed by \citet{chen2020threshold}. 
% We do not do this in our experiments because at deployment time, it is often the case that discrete predictions are required.


==> Input_Files/Our_Metric_OLD.tex <==
\label{sec:our_metrix_exp}
 
Now we present our metric, \biasampours{}, which retains the desirable properties of \biasamptheirs{}, while addressing the
shortcomings noted in the previous section. To account for the need to disentangle the two possible directions of bias amplification (Sec.~\ref{sec:sub_disentangle}) the metric consists of two values, \biasampoursAT{} corresponding to the amplification of bias resulting from the protected attribute influencing the task prediction, and \biasampoursTA{}, corresponding to the amplification of bias resulting from the task influencing the protected attribute prediction. 
% Concretely, the metric is defined as:
Concretely, \biasampours{} is:
\begin{align}
    % \text{BiasAmp}_{\rightarrow} 
    \frac{1}{|\mathcal{A}||\mathcal{T}|}&
    \sum_{t\in \mathcal{T},a\in \mathcal{A}} 
    y(t,a)\Delta(t,a)  + (1-y(t,a))(-\Delta(t,a))
\label{eqn:oursfull} \\
% \end{align}
% where
% \textnormal{where }& \\
% \begin{align}
y(t,a) &= \mathbbm{1}\left [P(T_t=1,A_a=1) > P(T_t=1)P(A_a=1) \right] 
\label{eqn:oursy}\\
% \text{and } 
\Delta(t,a) &= \left\{
                \begin{array}{ll}
                  P(\hat{T}_t=1|A_a=1) - P(T_t=1|A_a=1) & \\ \text{if measuring }A \rightarrow T& \\
                  P(\hat{A}_a=1|T_t=1) - P(A_a=1|T_t=1) & \\\text{if measuring }T \rightarrow A&
                \end{array}
              \right.
\label{eqn:oursdiff}
% Z &= |\mathcal{A}| \text{ if measuring }A \rightarrow T \text{ and  } |\mathcal{T}| \text{ if measuring }T \rightarrow A
\end{align}

% \begin{align}
%     \text{BiasAmp}_{A\rightarrow T} &=\\   \frac{1}{|\mathcal{A}||\mathcal{T}|}&\sum_{t=1}^{|\mathcal{T}|} \left( \int_{thr}
%     \sum_{a=1}^{|\mathcal{A}|}  \left (
%     y(t,a)\Delta^{thr}(t,a)  + (1-y(t,a))(-\Delta^{thr}(t,a))   \right) \text{d}thr \right)
% \label{eqn:oursfull} \\
%     \text{BiasAmp}_{T\rightarrow A} &=\\   \frac{1}{|\mathcal{A}||\mathcal{T}|}&\sum_{a=1}^{|\mathcal{A}|} \left( \int_{thr} 
%     \sum_{t=1}^{|\mathcal{T}|}  \left (
%     y(t,a)\Delta^{thr}(t,a)  + (1-y(t,a))(-\Delta^{thr}(t,a))   \right) \text{d}thr \right)
% \label{eqn:oursfullother} \\
% \text{where } 
% y(t,a) &= \mathbbm{1}\left [P(T_t=1,A_a=1) > P(T_t=1)P(A_a=1) \right] 
% \label{eqn:oursy}\\
% % \text{and } 
% \Delta^{thr}(t, a) &= \left\{
%                 \begin{array}{ll}
%                   P(\hat{T}^{thr}_t=1|A_a=1) - P(T_t=1|A_a=1) & \text{if measuring }A \rightarrow T \\
%                   P(\hat{A}^{thr}_a=1|T_t=1) - P(A_a=1|T_t=1) & \text{if measuring }T \rightarrow A
%                 \end{array}
%               \right.
% \label{eqn:oursdiff}
% % Z &= |\mathcal{A}| \text{ if measuring }A \rightarrow T \text{ and  } |\mathcal{T}| \text{ if measuring }T \rightarrow A
% \end{align}


% Note that $\hat{T}_t^{thr}$ and $\hat{A}_a^{thr}$ correspond to the predictions of the task and protected attribute respectively under a classification threshold $thr$. 
% The metric addresses the shortcomings described in Sec.~\ref{sec:biasamptheirs} along with a few additional modifications. 
Eqn.~\ref{eqn:oursfull} 
generalizes \biasamptheirs{} to measure the amplification of both 
positive and negative correlations between task $T_t$ and attribute $A_a$ when the attributes are non-binary, as discussed in Sec.~\ref{sec:nonbinary}. Eqn.~\ref{eqn:oursy} identifies the direction of correlation of attribute $A_a$ with task $T_t$, properly accounting for base rates as described in Sec.~\ref{sec:baserates}. Finally, Eqn.~\ref{eqn:oursdiff} decouples the two possible directions of bias amplification as in Sec.~\ref{sec:sub_disentangle}. Since values may be negative, reporting the aggregated bias amplification value could obscure task-attribute pairs that exhibit strong bias amplification; thus, disaggregated results per pair can be returned.
% for a more detailed diagnosis

% Although in much of the examples we have and will look at, $\mathcal{A}=\{\text{woman}, \text{man}\}$, this formulation allows for any attribute set to be defined, including intersectional identities. This is achieved by having $\mathcal{A}$ encompass the cross-product of possible attributes, for example $\mathcal{A}=\{\text{Black woman}, \text{Black man}, \text{white woman}, \text{white man}\}$.

% \subsection{Directions for Mitigation}
% \label{sec:mitigation}

% \begin{figure}
% \centering
% \centering
%   \centering
%   \includegraphics[width=.8\linewidth]{Images/coco_masks.png}
%   \caption{\biasampours{} of three conditions of images: full, noisy person mask, full person mask. As less of the person is visible, A$\rightarrow$T decreases from less human attribute visual cues to bias the task prediction. T$\rightarrow$A increases as the model relies on visual cues from the task to predict the attribute.}
%   \label{fig:coco_mask}
% % \caption{A figure with two subfigures}
% % \label{fig:test}
% \end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=.6\linewidth]{Images/biasamp_by_prop.png}
% \caption{\label{fig:byprop}Bias amplification varying as a function of proportion of images classified to be men (changed with threshold).}
% \end{figure}

% \hspace{.02\textwidth}
\begin{table}
\includegraphics[width=.95\linewidth]{Images/coco_masks.png}
\caption{\biasampours{} changes as a result of three conditions of images: full, noisy person mask, full person mask. As less of the person is visible, A$\rightarrow$T decreases from less human attribute visual cues to bias the task prediction. T$\rightarrow$A increases because the model must rely on visual cues from the task to predict the attribute.}
  \label{fig:coco_mask}
% \caption{A figure with two subfigures}
% \label{fig:test}
\end{table}

% \smallsec{Disentangling Directions}
We introduce a scenario for validating the decoupling aspect of our metric, that simultaneously serves as inspiration for an intervention approach to mitigating bias amplification. We use a baseline amplification removal idea of applying segmentation masks (noisy or full) over the people in an image to mitigate bias stemming from human attributes~\citep{wang2019balanced}. We train on the COCO classification task, with the same 66 objects from~\citet{zhao2017menshop}, a VGG16~\citep{simonyan2014vgg} model pretrained on ImageNet~\citep{imagenet} to predict objects and gender, with a Binary Cross Entropy Loss over all outputs, and measure \biasampoursTA{} and \biasampoursAT{}; we report 95\% confidence intervals for 5 runs of each scenario. In Tbl.~\ref{fig:coco_mask} we see, as expected, that as less of the person is visible, A$\rightarrow$T decreases because there are less human attribute visual cues to bias the task prediction. On the other hand, T$\rightarrow$A increases because the model must lean into task biases to predict the person's attribute. However, we can also see from the overlapping confidence intervals that the difference between noisy and full masks does not
% that this technique of bias amplification mitigation does not 
appear to be particularly robust; we continue a discussion of this phenomenon in Sec.~\ref{sec:consistency}.
Further mitigation techniques are outside of our scope, but we look to works like~\citet{singh2020context, wang2019balanced, agarwal2020spurious}.
